Neutrinos, Cosmic Rays and the MeV Band

The possible association of the blazar TXS 0506+056 with a high-energy neutrino detected by IceCube holds the tantalizing potential to answer three astrophysical questions: 1. Where do high-energy neutrinos originate? 2. Where are cosmic rays produced and accelerated? 3. What radiation mechanisms produce the high-energy {\gamma}-rays in blazars? The MeV gamma-ray band holds the key to these questions, because it is an excellent proxy for photo-hadronic processes in blazar jets, which also produce neutrino counterparts. Variability in MeV gamma-rays sheds light on the physical conditions and mechanisms that take place in the particle acceleration sites in blazar jets. In addition, hadronic blazar models also predict a high level of polarization fraction in the MeV band, which can unambiguously distinguish the radiation mechanism. Future MeV missions with a large field of view, high sensitivity, and polarization capabilities will play a central role in multi-messenger astronomy, since pointed, high-resolution telescopes will follow neutrino alerts only when triggered by an all-sky instrument.

==> Definitions/journalnames.tex <==
\DeclareOption{ArXiv}{ 	    \gdef\@journal{ArXiv}	\gdef\@journalshort{ArXiv}	\gdef\@journalfull{ArXiv}	\gdef\@doiabbr{ArXiv}	}
